Cross-Modal Contrastive Learning for Text-to-Image Generation

The output of text-to-image synthesis systems should be coherent, clear, photo-realistic scenes with high semantic fidelity to their conditioned text descriptions. Our Cross-Modal Contrastive Generative Adversarial Network (XMC-GAN) addresses this challenge by maximizing the mutual information between image and text. It does this via multiple contrastive losses which capture inter-modality and intra-modality correspondences. XMC-GAN uses an attentional self-modulation generator, which enforces strong text-image correspondence, and a contrastive discriminator, which acts as a critic as well as a feature encoder for contrastive learning. The quality of XMC-GAN's output is a major step up from previous models, as we show on three challenging datasets. On MS-COCO, not only does XMC-GAN improve state-of-the-art FID from 24.70 to 9.33, but--more importantly--people prefer XMC-GAN by 77.3 for image quality and 74.1 for image-text alignment, compared to three other recent models. XMC-GAN also generalizes to the challenging Localized Narratives dataset (which has longer, more detailed descriptions), improving state-of-the-art FID from 48.70 to 14.12. Lastly, we train and evaluate XMC-GAN on the challenging Open Images data, establishing a strong benchmark FID score of 26.91.

==> figures/ablation_tables.tex <==
\begin{table}[t]
\begin{center}
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccccccc}
\hline
\textbf{S} & \textbf{W} & \textbf{I} & \textbf{IS} $\uparrow$ & \textbf{FID} $\downarrow$  & \textbf{R-prec} $\uparrow$ & \textbf{SOA-C} $\uparrow$ & \textbf{SOA-I} $\uparrow$ \\
\hline
 \multicolumn{3}{c}{Real Images~\cite{hinz2020semantic}} & 34.88 & \pz 6.09 & 69.36 & 76.17 & 80.12 \\
\hline
 & & & 15.89 & 39.28 & 21.41 & 8.99 & 25.72  \\
 %baseline
 \checkmark & & & 23.50 & 19.25 & 53.57 & 24.57 & 45.41  \\ % sentence
 & \checkmark & & 20.72 & 24.38 & 44.42 & 20.50 & 39.12  \\ % word
 & & D &  18.90 & 29.71 & 31.16 & 12.73 & 30.89 \\ % G only
 & & VGG & 21.54 & 39.58 & 35.89 & 17.41 & 35.08  \\ % VGG
 & & D + VGG & 23.61 & 21.14 & 47.04 & 23.87 & 44.41  \\ % D + VGG  % TODO: update experiment 7 from xm2a/experiments/18601489
 \checkmark & \checkmark & &  26.02 & 14.25 & 64.94 & 30.49 & 51.60  \\  % word + sent
 \checkmark & \checkmark & D & 28.06 & 12.96 & 65.36 & 34.21 & 54.23  \\ % sent + word + D
 \checkmark & \checkmark & VGG & 30.55 & \textbf{11.12} & \textbf{70.98} & 39.36 & 59.10  \\ % sent + word + VGG 
\checkmark & \checkmark & D + VGG & \textbf{30.66} & 11.93 & 69.86 & \textbf{39.85} & \textbf{59.78}  \\ % word + sent + G + VGG 
\hline
\end{tabular}
}
\end{center}
\vspace{-10pt}
\caption{Ablation results with different contrastive losses on \cocoold. \textbf{S} indicates the sentence-image loss. \textbf{W} indicates the region-word loss. \textbf{I} indicates the image-image loss, where D represents using the discriminator to extract image features, and VGG represents using a pre-trained VGG network to extract image features.}
%All metrics are computed over 30,000 random samples using metrics re-implementated in TensorFlow.}
\vspace{-10pt}
\label{tab:ablation_2014}
\end{table}

% \begin{table*}[t]
% \begin{center}
% %\normalfont
% %\scriptsize
% % \footnotesize
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{l@{\hspace{8mm}}c@{\hspace{5mm}}c@{\hspace{5mm}}c@{\hspace{5mm}}c@{\hspace{5mm}}c@{\hspace{5mm}}c@{\hspace{5mm}}c@{\hspace{5mm}}c@{\hspace{5mm}}}
% \hline
% \textbf{Model} & \textbf{Sentence} & \textbf{Word} & \textbf{Image} & \textbf{IS} $\uparrow$ & \textbf{FID} $\downarrow$  & \textbf{\rprec} $\uparrow$ & \textbf{SOA-C} $\uparrow$ & \textbf{SOA-I} $\uparrow$ \\
% \hline
% Real Images~\cite{hinz2020semantic} & & & & 34.88 & \pz 6.09 & 69.36 & 76.17 & 80.12 \\
% \hline
%  &  &  &  & 15.89 & 39.28 & 21.41 & 8.99 & 25.72  \\
%  %baseline
%  & \checkmark & & & 23.50 & 19.25 & 53.57 & 24.57 & 45.41  \\ % sentence
%  & & \checkmark & & 20.72 & 24.38 & 44.42 & 20.50 & 39.12  \\ % word
%  & & & D &  18.90 & 29.71 & 31.16 & 12.73 & 30.89 \\ % G only
% & & & VGG & 21.54 & 39.58 & 35.89 & 17.41 & 35.08  \\ % VGG
% & & & D + VGG & 23.61 & 21.14 & 47.04 & 23.87 & 44.41  \\ % D + VGG  % TODO: update experiment 7 from xm2a/experiments/18601489
%  & \checkmark & \checkmark & &  26.02 & 14.25 & 64.94 & 30.49 & 51.60  \\  % word + sent
%  & \checkmark & \checkmark & D & 28.06 & 12.96 & 65.36 & 34.21 & 54.23  \\ % sent + word + D
%  & \checkmark & \checkmark & VGG & 30.55 & \textbf{11.12} & \textbf{70.98} & 39.36 & 59.10  \\ % sent + word + VGG 
% \CLGAN & \checkmark & \checkmark & D + VGG & \textbf{30.66} & 11.93 & 69.86 & \textbf{39.85} & \textbf{59.78}  \\ % word + sent + G + VGG 
% \hline
% \end{tabular}
% }
% \end{center}
% \vspace{-6pt}
%     \caption{Ablation results with different contrastive losses on \cocoold (256px images).}
% % \vspace{-10pt}
% \label{tab:ablation_2014} 
% \end{table*}



==> figures/coco_compare.tex <==
\begin{figure*}
\small
\begin{center}
\begin{tabular}{>{\arraybackslash}m{0.1\linewidth}@{\hskip 0.5em}c@{\hskip 0.1em}c@{\hskip 0.1em}c@{\hskip 0.1em}c@{\hskip 0.2em}|>{\arraybackslash}m{0.2\linewidth}@{\hskip 0.5em}c@{\hskip 0.1em}c@{\hskip 0.1em}c@{\hskip 0.1em}}
\textbf{\coco Caption} & \textbf{OP-GAN} & \textbf{SD-GAN} & \textbf{CP-GAN} & \textbf{\CLGAN} & \textbf{\cocoln Caption} & \textbf{AttnGAN} & \textbf{TReCS} & \textbf{\CLGAN} \\ \midrule \addlinespace[-0.05em]
\compareexamplesmall{a green train is coming down the tracks}{COCO_val2014_000000000923} &
\compareexamplelnnooriginal{There is a group of people. They are standing on ski board. They are smiling. They are holding a sticks. In the center of the person is wearing a helmet. On the right side ...}{470779_71}{000000470779} \\
\compareexamplesmall{A group of skiers are preparing to ski down a mountain.}{COCO_val2014_000000000761} &
\compareexamplelnnooriginal{In this image I can see people are sitting on chairs. I can also see few of them are wearing shades. Here I can see few more chairs and tables. On this table I can see food ...}{470924_85}{000000470924} \\
\compareexamplesmall{A small kitchen with low a ceiling}{COCO_val2014_000000000164} &
\compareexamplelnnooriginal{This picture shows an inner view of a restroom we see a wash basin with tap and a mirror on the wall and we see a light on it and we see a toilet seat and a frame on the wall and ...}{489091_37}{000000489091} \\\addlinespace[0.1em]
\compareexamplesmall{A child eating a birthday cake near some balloons.}{COCO_val2014_000000000428} &
\compareexamplelnnooriginal{In this image we can see a red color train on the railway track. Here we can see platform}{539445_12}{000000539445} \\
\compareexamplesmall{A living area with a television and a table}{COCO_val2014_000000000139} &
\compareexamplelnnooriginal{In this picture there are two members lying on the beach in the sand under an umbrella. There are some people standing here. In the background there is water}{262048_39}{000000262048} \\

\end{tabular}
\end{center}
\vspace{-10pt}
\caption{Generated images for selected examples from \cocoold and \cocoln. \CLGAN generated images are generally of much higher quality and depict clearer scenes. More random samples are available in the appendix.} \label{fig:compare_coco}
\end{figure*}

% \begin{figure*}
% \small
% \begin{center}
% \begin{tabular}{>{\arraybackslash}m{0.1\linewidth}@{\hskip 0.5em}c@{\hskip 0.1em}c@{\hskip 0.1em}c@{\hskip 0.1em}c@{\hskip 0.1em}>{\arraybackslash}m{0.1\linewidth}@{\hskip 0.5em}c@{\hskip 0.1em}c@{\hskip 0.1em}c@{\hskip 0.1em}c@{\hskip 0.1em}}
% %\toprule
%  \textbf{Caption} & \textbf{OP-GAN} & \textbf{SD-GAN} & \textbf{CP-GAN} & \textbf{\CLGAN} & \textbf{Caption} & \textbf{OP-GAN} & \textbf{SD-GAN} & \textbf{CP-GAN} & \textbf{\CLGAN} \\ \midrule

% \compareexamplesmall{a green train is coming down the tracks}{COCO_val2014_000000000923} &
% \compareexamplesmall{A group of men on a field playing baseball.}{COCO_val2014_000000000357} \\
% \compareexamplesmall{A group of skiers are preparing to ski down a mountain.}{COCO_val2014_000000000761} &
% \compareexamplesmall{A man sitting under a sun umbrella by an industrial port}{COCO_val2014_000000001244} \\
% \compareexamplesmall{A small kitchen with low a ceiling}{COCO_val2014_000000000164} &
% \compareexamplesmall{a white boat is out on the water}{COCO_val2014_000000000400} \\
% % \compareexamplesmall{An airplane approaching for landing over the water.}{COCO_val2014_000000000472} &
% % \compareexamplesmall{This table is filled with a variety of different dishes.}{COCO_val2014_000000000196} \\
% \compareexamplesmall{A child eating a birthday cake near some balloons.}{COCO_val2014_000000000428} &
% \compareexamplesmall{A large bear that is sitting on grass.}{COCO_val2014_000000000285} \\
% \compareexamplesmall{A living area with a television and a table}{COCO_val2014_000000000139} &
% \compareexamplesmall{A man throwing a frisbee in a dark field.}{COCO_val2014_000000000589} \\
% % \compareexamplesmall{A giraffe walking across a lush green field.}{COCO_val2014_000000001063} &
% % \compareexamplesmall{A woman posing for the camera standing on skis.}{COCO_val2014_000000000785} \\
% % \compareexamplesmall{A man displaying pots and utensils on a wall.}{COCO_val2014_000000000294} &
% % \compareexamplesmall{A baseball game is going on for the crowd.}{COCO_val2014_000000000544} \\
% % \compareexamplesmall{A group of elephants walking in muddy water.}{COCO_val2014_000000000757} &
% % \compareexamplesmall{a huge building with a four sided clock}{COCO_val2014_000000000626} \\

% \end{tabular}
% \end{center}
% \vspace{-10pt}
% \caption{Generated images for selected examples from \cocoold. \CLGAN generated images are generally of much higher quality and depict clearer scenes. More random samples are available in the supplementary material.} \label{fig:compare_coco}
% \end{figure*}

==> figures/compare_table.tex <==
\begin{table*}
\begin{center}
%\small
%\normalfont
%\scriptsize
% \footnotesize
\resizebox{0.7\linewidth}{!}{%
\begin{tabular}{l@{\hspace{8mm}}c@{\hspace{4mm}}c@{\hspace{4mm}}c@{\hspace{4mm}}c@{\hspace{4mm}}c@{\hspace{4mm}}}
\hline
\textbf{Model}  & \textbf{IS} $\uparrow$ & \textbf{FID} $\downarrow$ & \textbf{R-prec (CC) $\uparrow$} & \textbf{SOA-C} $\uparrow$ & \textbf{SOA-I} $\uparrow$ \\
\hline
Real Images & 34.88 & 6.09 & 69.36 & 74.97 & 80.84 \\
\hline
AttnGAN \cite{xu18} & 23.61 & 33.10 & - & 25.88 & 39.01 \\
Obj-GAN \cite{objgan19} & 24.09 & 36.52 & - & 27.14 & 41.24 \\
DM-GAN \cite{zhu2019dm} & 32.32 & 27.34 & - & 33.44 & 48.03 \\ 
OP-GAN \cite{hinz2020semantic} & 27.88 & 24.70 & 49.80 & 35.85 & 50.47 \\
SD-GAN \cite{yin2019semantics} & 35.69 & \pz29.35$^\dagger$ & 51.68 & - & - \\
CP-GAN \cite{liang2019cpgan} & \textbf{52.73} & \pz55.82$^\ddagger$ & 59.05 & \textbf{77.02} & \textbf{84.55} \\
\CLGAN (ours) & 30.45 & \pz\textbf{9.33} & \textbf{71.00} & 50.94 & 71.33 \\
\hline
\end{tabular}
}
\end{center}
\vspace{-10pt}
\caption{Comparison of \CLGAN with previous models on \cocoold. \textit{R-prec (CC)} are R-precision scores computed from a model trained on Conceptual Captions (see Sec.~\ref{sec:evaluation}). $^\dagger$ indicates scores computed from images shared by the original paper authors, and $^\ddagger$ indicates scores computed from images generated from the open-sourced models.}
% \vspace{-10pt}
\label{tab:compare_others}
\vspace*{-0.2in}
\end{table*}


% \begin{table*}
% \begin{center}
% %\normalfont
% %\scriptsize
% % \footnotesize
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{l@{\hspace{8mm}}c@{\hspace{5mm}}c@{\hspace{5mm}}c@{\hspace{5mm}}c@{\hspace{5mm}}c@{\hspace{5mm}}c@{\hspace{5mm}}}
% \hline
% \textbf{Model}  & \textbf{IS} $\uparrow$ & \textbf{FID} $\downarrow$ & \textbf{\rprec} $\uparrow$ & \textbf{\rprec (CC) $\uparrow$} & \textbf{SOA-C} $\uparrow$ & \textbf{SOA-I} $\uparrow$ \\
% \hline
% Real Images & 34.88 & 6.09 & 68.58 & 69.36 & 74.97 & 80.84 \\
% \hline
% AttnGAN \cite{xu18} & 23.61 & 33.10 & 83.80 & - & 25.88 & 39.01 \\
% Obj-GAN \cite{objgan19} & 24.09 & 36.52 & 87.84 & - & 27.14 & 41.24 \\
% DM-GAN \cite{zhu2019dm} & 32.32 & 27.34 & 91.87 & - & 33.44 & 48.03 \\ 
% OP-GAN \cite{hinz2020semantic} & 27.88 & 24.70 & 89.01 & 49.80 & 35.85 & 50.47 \\
% SD-GAN \cite{yin2019semantics} & 35.69 & \pz29.35$^\dagger$ & - & 51.68 & - & - \\
% CP-GAN \cite{liang2019cpgan} & \textbf{52.73} & \pz55.82$^\dagger$ & - & 59.05 & \textbf{77.02} & \textbf{84.55} \\
% \CLGAN (ours) & 30.45 & \pz\textbf{9.33} & - & \textbf{71.00} & 50.94 & 71.33 \\
% \hline
% \end{tabular}
% }
% \end{center}
% \vspace{-10pt}
% \caption{Comparison of \CLGAN with previous models on \cocoold. \textit{\rprec} scores are computed from AttnGAN's DAMSM encoders; \textit{\rprec (CC)} scores are computed using a model trained on Conceptual Captions (see Sec.~\ref{sec:evaluation}). $^\dagger$ indicates scores computed from images generated from the open-sourced models or shared by the original paper authors.}
% % \vspace{-10pt}
% \label{tab:compare_others}
% \end{table*}

